BeACONS: A Blockchain-enabled Authentication and Communications Network for Scalable IoV

This paper introduces a novel blockchain-enabled authentication and communications network for scalable Internet of Vehicles, which aims to bolster security and confidentiality, diminish communications latency, and reduce dependence on centralised infrastructures like Certificate Authorities and Public Key Infrastructures by leveraging Blockchain-enabled Domain Name Services and Blockchain-enabled Mutual Authentication. The proposed network is structured into a primary layer, consisting of Road Side Units and edge servers as servers of Blockchain-enabled Domain Name Services for managing inter-vehicle communications identities, and a sub-layer within each vehicle for intra-vehicle communications via the Blockchain-enabled Mutual Authentication Protocol. This design facilitates secure connections across vehicles by coordinating between the layers, significantly improving communications security and efficiency. This study also evaluates Road Side Unit availability against the random distribution of Road Side Units along the route of different vehicles. The proposed model presents a novel pathway towards a decentralised, secure, and efficient Internet of Vehicles ecosystem, contributing to the advancement of autonomous and trustworthy vehicular networks.

==> scrapped.tex <==
In traditional PBFT, the client has no voice in choosing the primary node of a view which is decided entirely based on the interactions among the replicas. However, for IoV scenarios, a vehicle running on a road may drive out of service range of a RSU at any time, depending on factors like signal coverage. While the communication between this particular RSU out of the vehicle's reach and other RSUs may still be established, it cannot maintain stable and reliable communication with the vehicle. Meanwhile, the vehicle may have just driven into the service range of another RSU, which should be absorbed into the view as a new node. 

\subsubsection{Kick-out of a node out of range}
This is determined by the heartbeat of each node. Every node broadcasts heartbeat messages at pre-agreed upon intervals. The vehicle listens for these messages, records the identities of their senders and determine the total number. When a node is out of range and the latency becomes infinitely long, the vehicle just kicks it out of the network and sends a KICK message to the entire network. If other nodes can still connect to the to-be-kicked node, they assume that this is not a faulty node, but rather a node out of range. Per the vehicle's request, the rest of the nodes also kick it out of their network and update the new number of total nodes from the nodes' view. If the kicked-out node happens to be the primary node of the current view, then there comes a view change, and a new election has to be held. 

\subsubsection{Absorption of a new node coming into range}
When the vehicle receives the heartbeat of a new RSU, it sends an ABSORB request to all nodes in the network. If a consensus is reached among the nodes that they can connect to the node-to-be RSU, then the new node is officially absorbed into the network. Absorption of a new node does not cause a view change, unless the primary node happens to be leaving at the same time. 

In summary, the client (vehicle) has the right of veto over whether a node should stay in the view, and the right of recommending a new node for the network. 

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.



\begin{itemize}
    \item We introduced BeMutual into IoV as a user-centric, zero-trust, light-weight communication protocol for both inter- and intra- vehicle communication. By removing the need for Certificate Authority (CA) and Public Key Infrastructure (PKI), BeMutual enables User Equipment (UE) in IoV to establish encrypted, privacy-preserving P2P connections over wired or wireless channels, which are immune to common problems with centralised infrastructure such as expiration of CA certificates, faulty or malicious CA/PKI, etc. As a result, connection latency is reduced, which is critical to the latency-sensitive IoV. Issues exploiting bad communication identity authentication or lack of encryption including eavesdropping, impersonation, MITM, spoofing, sybil attacks, masquerading and injection are tackled, making IoV safer and more reliable. Because BeMutual consumes less computation resources than traditional encrypted protocols such as IKEv2 and TLS 1.3\cite{b5}, the system is made light-weight thus more suitable for microcomputers that are widely used in IoV. 
    \item We introduced BeDNS into IoV as an immutable decentralised name service for communication identity management. For inter- and intra-vehicle communication, we integrated into each area a unique BeDNS network, so holistically a multi-layer BeDNS is constructed. BeDNS guarantees secure routing and in-time update of routing information. 
    \item We integrated BeDNS nodes into RSUs to provide immediate BeDNS service for vehicles nearby. A relatively small number of nodes running on edge cloud servers in dedicated server rooms provide BeDNS service for other users off the road, and also serve as fallbacks for vehicles. This not only reduces latency in BeDNS services, but also mitigates the risk of nodes being out of service due to attacks such as DDoS. 
\end{itemize}



\begin{table}[htbp]
\caption{Access to SKs in the primary layer}
\begin{center}
\begin{tabular}{|l|l|}
\hline
\textbf{Category}& \textbf{SKs accessible to} \\
\cline{1-2} 
{Node} & {Operator/owner of the RSU/edge cloud server} \\ \hline
\multirow{2}{*}{Vehicle} & {Driver/owner of the vehicle} \\ 
\cline{2}
{Wireless communication modules of the vehicle} \\ 
\hline
{Others} & {Operator/owner} \\
\hline
\end{tabular}
\label{tab4}
\end{center}
\end{table}

I & M\{$BCADD_P$, ${ADD_{P}}$^{*}, ($BCADD_{Ui1}$, $ADD_{Ui1}$, $L_{Ui1}$)^{*}\}, T, S(M, T, {$SK_P$}, {$SK_{Ui1}$}^{*}, ...)



\begin{table*}[htbp]
\caption{Steps to establish a BeMutual connection in the sub-layer}
\begin{center}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c|l|}
\hline
\textbf{Step}& \textbf{Interaction} \\
1 & Alice $\rightarrow$ Bob: Auth Request\{$BCADD_B$, $ADD_A$, $PK_A$, $nonce_1$, ($ADD_A$, $nonce_1$)$SK_A$\}  \\ 
2 & Bob $\rightarrow$ Alice: Auth Response\{$BCADD_A$, $ADD_A$, $ADD_B$, $PK_B$, $nonce_2$, ($ADD_A$, $ADD_B$, $nonce_2$)$SK_B$\} \\ 
3 & Alice $\rightarrow$ Bob: Session Key\{$BCADD_B$, $ADD_B$, $ADD_A$, ($KeyMaterial$)$PK_B$ \} \\
\hline
\end{tabular}
\label{tab6}
\end{center}
\end{table*}

\subsection{When a vehicle enters the network}
As is shown in Fig x, RSUs Nx in service constantly broadcast their BCADD and public key {BCADD Nx, PK Nx}. Vehicle Vy running on the road listen for such broadcast information and respond with {BCADD Nx, BCADD Vy, PK Vy, nonce1, (BCADD Vy, nonce1) SK Vy}. ......then the connection is established. 

Once the connection is established, the vehicle updates its network interface information. 

(Let\(\sqrt{R^{2}-\left(vt-y\right)^{2}}\)be noted as a,\(\frac{z+\sqrt{2R^{2}-z^{2}}}{2}\)be noted as p,\(\frac{z-\sqrt{2R^{2}-z^{2}}}{2}\)be noted as q)

\begin{equation}\left(z\geq\sqrt{2}R,vt\leq z,vt\leq2R\right)\end{equation}
\begin{equation}P=2\int_{n-R}^{\frac{nt}{2}}\int_{-a}^{a}f(x)dxdy\end{equation}
\begin{equation}\left(z\geq\sqrt{2}R,vt>z,vt-z\leq2\sqrt{R^{2}-\frac{z^{2}}{4}}\right)\end{equation}
\begin{equation}P=2\int_{z-R}^{\frac{z}{2}}\int_{-a+\nu t-z}^{a}f(x)dxdy\end{equation}

(We have \(\int_{\nu t-R}^{\frac{\nu t}{2}}\int_{-\mathrm{a}}^{\mathrm{a}}f(x)dxdy\)=A

\(\int_{\mathrm{p}}^{R}\int_{-\sqrt{R^{2}-y^{2}}}^{\sqrt{R^{2}-y^{2}}}f(x)dxdy\)=B

\(\int_{\mathrm{q}}^{\mathrm{p}}\int_{z-\sqrt{R^2-y^2}}^{y}f(x)dxdy\)=C)

\begin{equation}\left(z\geq R,\nu t\leq z,\nu t\leq z-\sqrt{2R^2-z^2}\right)\end{equation}
\begin{equation}P=\mathrm{A}+\int_{\frac{\nu t}{2}}^{\mathrm{q}}\int_{-\sqrt{R^2-y^2}}^{\sqrt{R^2-y^2}}f(x)dxdy+\int_{\mathrm{q}}^{\mathrm{p}}\int_{-\sqrt{R^2-y^2}}^{z-y}f(x)dxdy+\mathrm{B}+C\end{equation}

\begin{equation}
\left(z\geq R,\nu t\leq z,\nu t>z-\sqrt{2R^2-z^2}\right)
\end{equation}

\begin{align*}
P = & \int_{v-R}^{q}\int_{-a}^{a}f(x) \, dx \, dy \\
& + \int_{q}^{\frac{vt}{2}}\int_{-a}^{y-z}f(x) \, dx \, dy \\
& + \int_{\frac{vt}{2}}^{p}\int_{-\sqrt{R^{2}-y^{2}}}^{z-y}f(x) \, dx \, dy \\
& + \mathrm{B} + \mathrm{C} \\
& + \int_{q}^{R}\int_{z-\sqrt{R^{2}-y^{2}}}^{z-xt+\sqrt{R^{2}-y^{2}}}f(x) \, dx \, dy
\end{align*}


\(\left(z\geq R,\nu t>z,\nu t\leq z-\sqrt{2R^{2}-z^{2}}\right)\)

\begin{align*}
P = & \mathrm{A} + \int_{\frac{\nu t}{2}}^{\mathrm{q}}\int_{-\sqrt{R^{2}-y^{2}}+\nu t-z}^{\sqrt{R^{2}-y^{2}}} f(x) \, dx \, dy \\
& + \int_{\mathrm{q}}^{\mathrm{p}}\int_{-\sqrt{R^{2}-y^{2}}+\nu t-z}^{z-y} f(x) \, dx \, dy \\
& + \mathrm{B} + \mathrm{C}
\end{align*}

\begin{equation}\left(z\geq R,\nu t>z,\nu t>z-\sqrt{2R^2-z^2}\right)\end{equation}
\begin{align*}
P = & A + \int_{\frac{vt}{2}}^{q}\int_{-\sqrt{R^2-y^2}+vt-z}^{\sqrt{R^2-y^2}} f(x) \, dx \, dy \\
& + \int_{q}^{p}\int_{-\sqrt{R^2-y^2}+vt-z}^{z-y} f(x) \, dx \, dy \\
& + B + \int_{q+vt-z}^{p}\int_{z-\sqrt{R^2-y^2}}^{y} f(x) \, dx \, dy \\
& + \int_{q}^{q+vt-z}\int_{z-\sqrt{R^2-(vt-z-y)^2}}^{y} f(x) \, dx \, dy
\end{align*}

(Let \( f(x) \) denote the probability density function distributed along the roadway, where \( x \) represents the distance from the road, \( y \) signifies the distance of the vehicle from the initial position at a certain moment, \( z \) stands for the distance from the intersection, \( v \) denotes the vehicle speed, \( t \) represents the required time, and \( R \) represents the radius.)

\begin{thebibliography}{00}
\bibitem{b1} H. Taslimasa, S. Dadkhah, E. C. P. Neto, P. Xiong, S. Ray, and A. A. Ghorbani, “Security issues in Internet of Vehicles (IoV): A comprehensive survey,” Internet of Things, p. 100809, May 2023, doi: https://doi.org/10.1016/j.iot.2023.100809.

\bibitem{b2} A. Alnasser, H. Sun, and J. Jiang, “Cyber security challenges and solutions for V2X communications: A survey,” Computer Networks, vol. 151, pp. 52–67, Mar. 2019, doi: https://doi.org/10.1016/j.comnet.2018.12.018.

\bibitem{b3} S. Sharma and B. Kaushik, “A survey on internet of vehicles: Applications, security issues & solutions,” Vehicular Communications, vol. 20, p. 100182, Sep. 2019, doi: https://doi.org/10.1016/j.vehcom.2019.100182.
‌
\bibitem{b4} Z. El-Rewini, K. Sadatsharan, D. F. Selvaraj, S. J. Plathottam, and P. Ranganathan, “Cybersecurity challenges in vehicular communications,” Vehicular Communications, vol. 23, p. 100214, Jun. 2020, doi: https://doi.org/10.1016/j.vehcom.2019.100214.
\bibitem{b5} H. Xu, L. Zhang, Y. Sun, and C.-L. I, “BE-RAN: Blockchain-enabled Open RAN with Decentralized Identity Management and Privacy-Preserving Communication,” arXiv.org, May 29, 2021. https://arxiv.org/abs/2101.10856
\bibitem{b6} BE-DNS: Blockchain-enabled Decentralized Name
Services and P2P Communication Protocol
\bibitem{b7} “Securing Vehicle Electronic Control Unit (ECU) Communications and Stored Data - ProQuest,” www.proquest.com. https://www.proquest.com/openview/59ef3de0f677eca3a40a7bb90188615a/1?pq-origsite=gscholar&cbl=18750 (accessed Apr. 10, 2024).
\bibitem{b8} H. Xiong, Z. Guan, Z. Chen, and F. Li, “An efficient certificateless aggregate signature with constant pairing computations,” Information Sciences, vol. 219, pp. 225–235, Jan. 2013, doi: https://doi.org/10.1016/j.ins.2012.07.004.
\bibitem{b9} An efficient certificateless aggregate signature with conditional
privacy-preserving for vehicular sensor networks
\bibitem{b10} An efficient certificateless aggregate signature without pairings for vehicular ad hoc networks
\bibitem{b11} An improved certificateless aggregate signature scheme without bilinear pairings for vehicular ad hoc networks
\bibitem{b12} Y. Zhao, Y. Hou, L. Wang, S. Kumari, M. K. Khan, and H. Xiong, “An efficient certificateless aggregate signature scheme for the Internet of Vehicles,” Transactions on Emerging Telecommunications Technologies, vol. 31, no. 5, Aug. 2019, doi: https://doi.org/10.1002/ett.3708.
\bibitem{b13} Efficient and Secure Certificateless Signcryption Without Pairing for Edge Computing-Based Internet of Vehicles
\bibitem{b14} ELCPAS: A new efficient lightweight certificateless conditional privacy preserving authentication scheme for IoV
\bibitem{b15} A Secured and Efficient Communication Scheme for Decentralized Cognitive Radio-Based Internet of Vehicles
\bibitem{b16} Blockchain for the Internet of Vehicles: A Decentralized IoT Solution for Vehicles Communication Using Ethereum
\bibitem{b17} LBSV: Lightweight Blockchain Security Protocol for Secure Storage and Communication in SDN-Enabled IoV
\end{thebibliography}



distance between the vehicle and each RSU is changing all the time. During this process, connections between some of the RSUs and the vehicle drop because either side leaves the wireless coverage zone of the other side. Meanwhile, some other RSUs become available as they come into service range. The availability of an RSU is signalled by regularly broadcasting heartbeat messages containing its g-BCADD. Once the vehicle successfully captures a heartbeat message sent by an RSU to which the vehicle is not connected, the vehicle starts a BeMutual connection by sending this particular RSU an authentication request. When the connection is lost, the vehicle will make several attempts to reconnect and will keep listening for heartbeat messages of the RSU in the meantime before eventually identifying this RSU as an out-of-range one and terminating further attempts to reconnect. During the available time slot (ATS) of the RSU, it provides for the vehicle services including but not limited to BeDNS, all over the secure BeMutual protocol. 


\begin{algorithm}
\caption{Absorption of new RSU}\label{absorption}
\begin{algorithmic}[1]
\Procedure{Absorption}{}
    \If{reception of heartbeat of new RSU $X_n$ at $V$} 
    \State $V$ start BeMutual Authentication with $X_n$
    \If{BeMutual session is established}
    \State $V$ sends request of absorption of $X_n$ $Req_{Abs}$($X_n$) to $X_p$
    \If{PBFT consensus in G on $Req_{Abs}$($X_n$) is reached}
    \State $N_{Xi} \gets N_{Xi} + 1$
    \State $X_i$ executes $Abs(X_n)$
    \State $X_i$ sends reply $Rpl_{Abs}$($X_n$) to $V$
    \If{reception of $\left(\frac{N_v+2}{3}\right)$ $Rpl_{Abs}$($X_n$) at $V$}
    \State $V$ executes $Ack_{Abs}$($X_n$)
    \State $N_{V} \gets N_{V} + 1$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Expulsion of an RSU out of range}\label{expulsion}
\begin{algorithmic}[1]
\Procedure{Expulsion}{}
    \If{$V$ loses heartbeat of RSU $X_n$} 
    \State $V$ broadcasts to $X_i$ request of expulsion of $X_n$ $Req_{Exp}$($X_n$)
    \If{PBFT consensus in G on $Req_{Exp}$($X_n$) is reached}
    \If{$X_n$ is $X_p$}
    \State view change $VC$($X_p$) is executed
    \State $X_i$' executes $Exp(X_n)$
    \State $N_{Xi'} \gets N_{Xi'} - 1$
    \State $X_i$' sends reply $Rpl_{Exp}$($X_n$) to $V$
    \Else $X_i$ executes $Exp(X_n)$
    \State $N_{Xi} \gets N_{Xi} - 1$
    \State $X_i$ sends reply $Rpl_{Exp}$($X_n$) to $V$
    \If{reception of $\left(\frac{N_v+1}{3}\right)$ $Rpl_{Exp}$($X_n$) at $V$}
    \State $V$ executes $Ack_{Exp}$($X_n$)
    \State $N_{V} \gets N_{V} - 1$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsubsection{Within the Primary Layer}

\subsubsection{Between Vehicles and RSUs}
In this model, we assume that connections between vehicles and RSUs are physically P2P wireless connections. For these particular connections, the network interface identifier of each party are its own BCADD. Over such connections, vehicles connect to RSUs using the BeMutual protocol. BeDNS is not required in this process, because they are directly linked by default. After the connection is established, the vehicle updates mapping information (both CAT A and CAT B) concerning itself through smart contracts. 

As the vehicle keeps moving on the road, distance between the vehicle and each RSU is changing all the time. During this process, connections between some of the RSUs and the vehicle drop because either side leaves the wireless coverage zone of the other side. Meanwhile, some other RSUs become available as they come into service range. The availability of an RSU is signalled by regularly broadcasting heartbeat messages containing its g-BCADD. Once the vehicle successfully captures a heartbeat message sent by an RSU to which the vehicle is not connected, the vehicle starts a BeMutual connection by sending this particular RSU an authentication request. When the connection is lost, the vehicle will make several attempts to reconnect and will keep listening for heartbeat messages of the RSU in the meantime before eventually identifying this RSU as an out-of-range one and terminating further attempts to reconnect. During the available time slot (ATS) of the RSU, it provides for the vehicle services including but not limited to BeDNS, all over the secure BeMutual protocol. 

\subsubsection{Between Vehicles and Edge Cloud Servers}
Normally, edge-cloud-based nodes do not provide immediate BeDNS services for vehicles on the road. However, when a vehicle finds no available RSUs nearby but somehow still has Internet connection, edge cloud servers come into play as fallbacks. Unlike RSUs which constantly broadcast their g-BCADDs to nearby vehicles, edge cloud servers do not identify themselves proactively unless they receive an explicit request from a vehicle. Each vehicle keeps in its local storage a secure record of g-BCADDs and network interface identifiers of a certain number of available, trustworthy edge-cloud-based nodes. The record is regularly updated when the vehicle is connected either to RSUs or to edge cloud servers. 

\subsubsection{Between Vehicles}
Typically, Vehicles connect to one another using BeMutual protocol over wireless P2P links. However, in this model we also allow for scenarios in which vehicles have to connect through the Internet. BeMutual connections between vehicles have to go through smart contract verification on the blockchain. If two vehicles wish to be directly linked wirelessly, their network interface identifiers are their g-BCADDs. If they wish to connect through the Internet, then their network interface identifiers are their IP addresses. 

\subsubsection{Between Vehicles and Others}
These two parties connect in the same way that two vehicles do. 

\subsection{Inter-layer Interactions}
Often is the case that one Type I/II unit in a sub-layer wishes to connect to a Type III unit that is actually in another sub-layer or in the primary layer, or in reverse. For example, a car driving autonomously on the road requires direct links to sensors installed on neighbouring vehicles for better coordination. We define this type of interaction as inter-layer interactions. 

\subsubsection{Type I Unit as the Gateway}
For inter-layer interactions, at least one Type I unit has to be involved in order to relay the transmission from intra-vehicle network to inter-vehicle network and in reverse. This particular Type I unit is defined as the gateway of the sub-layer in which it is engaged. Typically, one vehicle can have many Type I units. A certain type of connection may have multiple available Type I units to choose from. A particular Type I unit may not support certain types of connection. However, they all have the same g-BCADD which is that of the vehicle. 

\subsubsection{Type I Unit as the Gateway}
For inter-layer interactions, at least one Type I unit has to be involved in order to relay the transmission from intra-vehicle network to inter-vehicle network and in reverse. This particular Type I unit is defined as the gateway of the sub-layer in which it is engaged. Typically, one vehicle can have many Type I units. A certain type of connection may have multiple available Type I units to choose from. A particular Type I unit may not support certain types of connection. However, they all have the same g-BCADD which is that of the vehicle. 

\subsubsection{Concatenated Global BCADDs (Cg-BCADDs) for units in a sub-layer}
To describe a unit in one sub-layer in a way that both participants in the primary layer and units in other sub-layers recognise, the concatenated global BCADD (Cg-BCADD) of the unit is introduced, which is the concatenation of the unit's sub-BCADD with the g-BCADD of the gateway of the sub-layer in which the unit is engaged, denoted by \textit{g-BCADD$_{gateway}$:sub-BCADD$_{unit}$}. 

\subsubsection{Adding CAT B Mapping Information to the Primary BeDNS}
Not all sensors in a vehicle should be shared with other vehicles, otherwise it poses not only security risks but also privacy concerns. Therefore, sensors not to be shared will not have their Cg-BCADDs uploaded to the primary blockchain, but rather keep them locally. Sensors to be shared update their mapping information regularly through the gateway. 

\subsubsection{Establishing Inter-layer BeMutual Connections}
For the most generalised part, if a Type II unit wishes to start a BeMutual connection with a Type III unit which is actually a Type II unit in another sub-layer, it has to connect to a Type I unit (gateway) in its sub-layer over BeMutual first. Using this gateway as a relay, the Type II unit then sends/receives requests of BeMutual connections and interacts with the primary BeDNS. Of course, if established, the inter-layer BeMutual connection is also relayed by Type I units. 

It is observed that the duration of RSUs' presence within the circular coverage area of vehicle signals, randomly distributed on both sides of the road, is solely determined by the distance \(d_1\) of the RSUs from the roadway.

In this scenario if RSUs remaining within the signal coverage area for a duration exceeding \(t\) are designated as effective RSUs, the number of effective RSUs within the signal coverage area of a vehicle traveling in a straight line can be worked out.

execute left or right turns, the duration of RSUs' presence within the signal coverage area in the vicinity of the turning angle is influenced by the distances \(d_1\) and \(d_2\) of the RSUs from the two roads.

At this juncture, the number of effective RSUs in the vicinity of a vehicle about to make a turn can be determined.

\subsection{Performance Analysis of BCADD Model}

We have configured a range of parameters to tailor our vehicular network for the multi-target analysis in the experiments, while also selecting specific performance indicators to investigate the outcomes.

Considering that the duration of RSUs staying in the vehicle communication coverage area varies during straight driving and turning processes, we set events every [ ] seconds in the simulation. In these events, vehicles have a certain probability of turning left, turning right, or going straight, resulting in representative and stochastic vehicle wandering routes. In each turning event, different vehicle types have different motion patterns, as detailed in the table. We will conduct separate simulation experiments for different vehicle types.


The mathematical expectation of effective RSUs within the signal coverage area per second (for taxi). Average: 5.376702







\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \textbf{Trial} & \textbf{Score} & \textbf{Trial} & \textbf{Score} & \textbf{Trial} & \textbf{Score} \\
        \hline
       1 & 4.044 & 18 & 4.3187 & 35 & 4.5824 \\
        2 & 4.1648 & 19 & 4.1648 & 36 & 4.1099 \\
        3 & 4.2857 & 20 & 4.2527 & 37 & 4.033 \\
        4 & 4.1429 & 21 & 4.6813 & 38 & 4.1099 \\
        5 & 4.1868 & 22 & 4.2637 & 39 & 4.1868 \\
        6 & 4.1209 & 23 & 4.3407 & 40 & 4.5385 \\
        7 & 4.044 & 24 & 4.011 & 41 & 4 \\
        8 & 5.1538 & 25 & 4.044 & 42 & 4.4615 \\
        9 & 4.4835 & 26 & 4.2198 & 43 & 4.8462 \\
        10 & 4.2637 & 27 & 3.7802 & 44 & 4.1868 \\
        11 & 3.8901 & 28 & 5.2418 & 45 & 4.5824 \\
        12 & 4.4066 & 29 & 4.1978 & 46 & 3.8462 \\
        13 & 4.1758 & 30 & 3.9011 & 47 & 4.4835 \\
        14 & 4.2637 & 31 & 4.044 & 48 & 4.5275 \\
        15 & 4.5714 & 32 & 4.022 & 49 & 4.2418 \\
        16 & 4.1758 & 33 & 3.7582 & 50 & 3.9341 \\
        17 & 4.7143 & 34 & 4.1209 & & \\
        \hline
    \end{tabular}
    \caption{Scores for van}
    \label{tab:scores_van}
\end{table}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.3\textwidth]{van.png}
    \caption{Van Image}
    \label{fig:van_image}
\end{figure}

\cite{Xiong2013} proposed a certificateless signature (CLS) scheme that is provably secure in the random oracle model under the standard Computational Diffe–Hellman (CDH) assumption. \cite{Horng2015} proposed a novel CLS scheme with a certificateless aggregate signature (CLAS) scheme for V2I communication. It implemented both certificateless public key cryptography and aggregate signature. 


\cite{Xu2021} proposed Blockchain-enabled Radio Access Networks (BE-RAN) as a novel decentralized RAN architecture that focuses on security and privacy of identification and authentication. It encompasses BeMutual as core functions of BE-RAN. Results show that BeMutual improves communication and computation overheads compared to the existing communication authentication protocols such as TLS 1.3 and IKEv2 protocols. 


\cite{Zhou2022} implemented BeDNS as a system of identity management integrated into Be-Mutual. BeDNS maps complicated blockchain addresses to simpler domain names and blockchain addresses to their owners' network interface identifiers, which serves as a secure verification method before establishing BeMutual connections. 


@article{Zhou2023,
   author = {Zihan Zhou and Chenxiao Guo and Hao Xu and Xiaoshuai Zhang and Yixuan Fan and Lei Zhang},
   title = {BE-DNS: Blockchain-enabled Decentralized Name Services and P2P Communication Protocol},
   year = {2023},
}


\begin{table}[h]
    \centering
    \caption{Average number of effective RSUs for taxi}
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \textbf{Trial} & \textbf{Avg.} & \textbf{Trial} & \textbf{Avg.} & \textbf{Trial} & \textbf{Avg.} \\
        \hline
       1 & 5.6264 & 18 & 7.3956 & 35 & 5.1319 \\
        2 & 4.8901 & 19 & 5.2637 & 36 & 4.7473 \\
        3 & 5.8571 & 20 & 4.4505 & 37 & 4.8462 \\
        4 & 5.9341 & 21 & 5.3516 & 38 & 6.2198 \\
        5 & 4.4725 & 22 & 4.4945 & 39 & 4.6813 \\
        6 & 5.2198 & 23 & 4.3187 & 40 & 4.978 \\
        7 & 4.9121 & 24 & 5.3846 & 41 & 4.8352 \\
        8 & 4.9341 & 25 & 5 & 42 & 5.3846 \\
        9 & 5.6593 & 26 & 6.4835 & 43 & 4.8352 \\
        10 & 6.1978 & 27 & 5.0549 & 44 & 5 \\
        11 & 5.6264 & 28 & 5.8681 & 45 & 7.044 \\
        12 & 4.9121 & 29 & 4.989 & 46 & 5.956 \\
        13 & 6.6484 & 30 & 4.4286 & 47 & 5.7802 \\
        14 & 6.3077 & 31 & 5.1868 & 48 & 5.1209 \\
        15 & 5.8681 & 32 & 5.4066 & 49 & 5.6264 \\
        16 & 5.8022 & 33 & 4.7802 & 50 & 5.1648 \\
        17 & 5.978 & 34 & 4.7802 & & \\
        \hline
    \end{tabular}
    \label{tab:scores_taxi}
\end{table}


\begin{table}[h]
    \centering
    \caption{Average number of effective RSUs for private car}
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \textbf{Trial} & \textbf{Avg.} & \textbf{Trial} & \textbf{Avg.} & \textbf{Trial} & \textbf{Avg.} \\
        \hline
        1 & 4.6703 & 18 & 4.4176 & 35 & 4.9121 \\
        2 & 4.6264 & 19 & 4.4615 & 36 & 5.2857 \\
        3 & 5.1538 & 20 & 4.7802 & 37 & 4.3297 \\
        4 & 6.6044 & 21 & 6.0769 & 38 & 5.5385 \\
        5 & 5.0879 & 22 & 4.2418 & 39 & 4.7692 \\
        6 & 4.6374 & 23 & 4.9231 & 40 & 5.011 \\
        7 & 4.8571 & 24 & 5.7033 & 41 & 4.1538 \\
        8 & 5.1978 & 25 & 4.1209 & 42 & 5.3626 \\
        9 & 4.4505 & 26 & 4.5604 & 43 & 4.5824 \\
        10 & 5.1648 & 27 & 4.3736 & 44 & 4.4505 \\
        11 & 5.1209 & 28 & 5.1209 & 45 & 4.1209 \\
        12 & 6.0659 & 29 & 5.022 & 46 & 4.5714 \\
        13 & 4.9341 & 30 & 4.7363 & 47 & 4.2967 \\
        14 & 5.1758 & 31 & 4.1758 & 48 & 4.3077 \\
        15 & 4.8022 & 32 & 5.3516 & 49 & 4.6264 \\
        16 & 4.7692 & 33 & 5.1099 & 50 & 4.1868 \\
        17 & 4.6703 & 34 & 4.5714 & & \\
        \hline
    \end{tabular}
    \label{tab:scores_private_car}
\end{table}


\begin{table}[h]
    \centering
    \caption{Average number of effective RSUs for van}
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \textbf{Trial} & \textbf{Avg.} & \textbf{Trial} & \textbf{Avg.} & \textbf{Avg.} & \textbf{Avg.} \\
        \hline
       1 & 4.044 & 18 & 4.3187 & 35 & 4.5824 \\
        2 & 4.1648 & 19 & 4.1648 & 36 & 4.1099 \\
        3 & 4.2857 & 20 & 4.2527 & 37 & 4.033 \\
        4 & 4.1429 & 21 & 4.6813 & 38 & 4.1099 \\
        5 & 4.1868 & 22 & 4.2637 & 39 & 4.1868 \\
        6 & 4.1209 & 23 & 4.3407 & 40 & 4.5385 \\
        7 & 4.044 & 24 & 4.011 & 41 & 4 \\
        8 & 5.1538 & 25 & 4.044 & 42 & 4.4615 \\
        9 & 4.4835 & 26 & 4.2198 & 43 & 4.8462 \\
        10 & 4.2637 & 27 & 3.7802 & 44 & 4.1868 \\
        11 & 3.8901 & 28 & 5.2418 & 45 & 4.5824 \\
        12 & 4.4066 & 29 & 4.1978 & 46 & 3.8462 \\
        13 & 4.1758 & 30 & 3.9011 & 47 & 4.4835 \\
        14 & 4.2637 & 31 & 4.044 & 48 & 4.5275 \\
        15 & 4.5714 & 32 & 4.022 & 49 & 4.2418 \\
        16 & 4.1758 & 33 & 3.7582 & 50 & 3.9341 \\
        17 & 4.7143 & 34 & 4.1209 & & \\
        \hline
    \end{tabular}
    \label{tab:scores_van}
\end{table}
